Advances and Challenges in Conversational Recommender Systems: A Survey

Recommender systems exploit interaction history to estimate user preference, having been heavily used in a wide range of industry applications. However, static recommendation models are difficult to answer two important questions well due to inherent shortcomings: (a) What exactly does a user like? (b) Why does a user like an item? The shortcomings are due to the way that static models learn user preference, i.e., without explicit instructions and active feedback from users. The recent rise of conversational recommender systems (CRSs) changes this situation fundamentally. In a CRS, users and the system can dynamically communicate through natural language interactions, which provide unprecedented opportunities to explicitly obtain the exact preference of users. Considerable efforts, spread across disparate settings and applications, have been put into developing CRSs. Existing models, technologies, and evaluation methods for CRSs are far from mature. In this paper, we provide a systematic review of the techniques used in current CRSs. We summarize the key challenges of developing CRSs in five directions: (1) Question-based user preference elicitation. (2) Multi-turn conversational recommendation strategies. (3) Dialogue understanding and generation. (4) Exploitation-exploration trade-offs. (5) Evaluation and user simulation. These research directions involve multiple research fields like information retrieval (IR), natural language processing (NLP), and human-computer interaction (HCI). Based on these research directions, we discuss some future challenges and opportunities. We provide a road map for researchers from multiple communities to get started in this area. We hope this survey can help to identify and address challenges in CRSs and inspire future research.

==> sections/removed-02-development.tex <==
\section{Development of Recommender Systems}
\label{sec:RS}

In this section, we briefly recall some common types of recommender systems, and we discuss some problems existing in these traditional models.

\subsection{Classic Recommendation Scenarios and Methods}
\Acp{RS} aim to learn users' preferences and provide suggestions for items or services they might consume. In terms of data requirements, earlier \ac{RS} algorithms can be divided into three paradigms \cite{balabanovic1997fab,adomavicius2005toward}: 
\begin{enumerate}[nosep,leftmargin=*]
\item \textbf{Content-based recommendations}, in which the system tries to recommend items similar to those a given user has liked in the past \cite{balabanovic1997fab}. For example, a man who always browses news with the keyword \emph{sports} is likely to accept recommendations about breaking sports news. 
Early implementation of content-based recommendation includes InfoFinder \cite{krulwich1996learning}, News\-Weed\-er \cite{lang1995newsweeder}, and systems developed for the routing task at the TREC conferences \cite{harman1995overview}. 
Most modern recommender systems in industry and aca\-demia combine other techniques because content-based recommendation has obvious shortcomings; e.g., it is hard to extract content-based features from items like movies and music. 
\item \textbf{\Acl{CF}.} Collaborative approaches refer to algorithms that provide item recommendations or predictions based on the opinions of other like-mind-ed users, which is also called user-based \acl{CF} \cite{CFshardanand1995social,CFresnick1994grouplens,schafer2007collaborative}. The opinions can be explicitly given by the user as a rating score, generally on a certain numerical scale, or they can be derived from purchasing records or by analyzing timing logs \cite{hu2008collaborative}. \citet{sarwar2001item} proposed item-based \acl{CF}; the intuition is that a user would be interested in purchasing items that are similar to the items the user liked earlier. \ac{CF} is the most prevalent setting in recommender systems. Common models include linear regression \cite{sarwar2001item}, Bayesian networks \cite{10.5555/2074094.2074100}, Markov decision processes \cite{shani2005mdp}, \ac{LDA}~\cite{marlin2004modeling}, clustering~\cite{basu1998recommendation,ungar1998clustering}, and rule-based approaches~\cite{sarwar2000analysis}. Matrix factorization-based \acl{CF} methods have dominated the recommendation community since they won the Netflix Prize \cite{koren2008factorization,10.1145/1557019.1557072,koren2009bellkor,MF}.  Collaborative approaches also have to encounter the cold-start and sparse problem. 

\item \textbf{Hybrid methods.} Some recommendation systems integrate the above two types of methods, thus the shortcomings can be alleviated \cite{Claypool1999CombiningCA,pazzani1999framework,tran2000hybrid,good1999combining,soboroff1999combining}.
\end{enumerate}

% \begin{itemize}
%   \item \textbf{Content-based recommendations.} In content-based recommendation, the system tries to recommend items similar to those a given user has liked in the past \cite{balabanovic1997fab}. For example, a man who always browsed news with the keyword \emph{sports} is likely to accept recommendations about breaking sport news. Furthermore, This branch of methods extend to explicitly considers users' profiles (e.g., age, occupation, and preferred keywords) and items' attributes (e.g., keywords, categories, brands), then match the certain group of users with items based on statistical rules. For example, the group of pregnant women might be interested in babies' clothes and milk powders. Early implement of content-based recommendations includes InfoFinder \cite{krulwich1996learning}, NewsWeeder \cite{lang1995newsweeder}, and systems developed for the routing task at the TREC conferences \cite{harman1995overview}. Most recommender systems in industry and academia consider combining other techniques, because content-based recommendation have obvious shortcomings, such as hard to extract content-based features from items like movies and musics, and it tends to recommend items similar to those users have already consumed. 

%   \item \textbf{\acl{CF} (CF).} Usually, collaborative approaches refer to algorithms that provide item recommendations or predictions based on the opinions of other like-minded users, which is also called user-based \acl{CF} \cite{CFshardanand1995social,CFresnick1994grouplens,schafer2007collaborative}. The opinions can be explicitly given by the user as a rating score, generally within a certain numerical scale, or can be implicitly derived from purchase records or by analyzing timing logs \cite{hu2008collaborative}. Then \citet{sarwar2001item} proposed item-based \acl{CF} of which the intuition is that a user would be interested in purchasing items that are similar to the items the user liked earlier. \citet{10.5555/2074094.2074100} further divide \acl{CF} algorithms into two categories–Memory-based and Model-based algorithms. Memory-based algorithms operate over the whole user dataset to find the neighbor users of the target user, then it makes recommendations according to these neighbor users' purchased history. Model-based algorithms, in contrast, develop a model to estimate user ratings on items. The common models include linear regression \cite{sarwar2001item}, Bayesian network \cite{10.5555/2074094.2074100}, Markov decision processes \cite{shani2005mdp}, Latent Dirichlet Allocation (LDA) \cite{marlin2004modeling}, clustering \cite{basu1998recommendation,ungar1998clustering}, and rule-based approaches \cite{sarwar2000analysis}. Matrix factorization-based \acl{CF} methods have dominated recommendation community since they won the Netflix Prize \cite{koren2008factorization,10.1145/1557019.1557072,koren2009bellkor,koren2009matrix}. Note that collaborative approaches also have to encounter the cold-start and sparse problem.

%   \item \textbf{Hybrid methods.} Some recommendation systems integrate above above two types of methods, so the shortcomings can be alleviated. According to the taxonomy of \citet{adomavicius2005toward}, there are four ways of combining collaborative and content-based methods: (1) implementing collaborative and content-based methods separately and combining their predictions \cite{Claypool1999CombiningCA,pazzani1999framework,tran2000hybrid}, (2) incorporating some content-based characteristics into a collaborative approach \cite{pazzani1999framework,balabanovic1997fab,good1999combining}, (3) incorporating some collaborative characteristics into a content-based approach \cite{soboroff1999combining}, and (4) constructing a general unifying model that incorporates both content-based and collaborative characteristics \cite{condli1999bayesian,ansari2000internet,10.5555/295240.295795,10.5555/2074022.2074076,hofmann1999probabilistic}. Note that most neural network-based methods belong to the fourth class, and we will discuss them later.
% \end{itemize}

\noindent
The methods listed above represent the most basic recommendation ideas or frameworks. However, real-world situations are complex, and no algorithm fits all scenarios. 
Based on the specific scenarios, many ad hoc algorithms have been proposed. For example, some common categories include context-aware recommendation \cite{verbert2012context,liu2013survey}, session-based (se\-quential) recommendation \cite{wang2019survey,soto2011temporal}, point-of-interest recommendation \cite{zhao2016survey}, deep-learning-based recommendation \cite{zhang2019deep}, and graph-learning-based recommendation \cite{yu2016network,wang2020graph}. 

% A lot of efforts have been made to research recommendation problems into different scenarios, which spawned many branches of different recommendation techniques. We select some works to review. 


% \begin{itemize}
%   \item \textbf{Context-aware Recommendation.} Given users' historical interactions on items, traditional recommender systems aim to capture the user preferences and predict users' ratings (a score) on certain items, then it makes recommendations using the items with the highest scores. However, in real-world situations, whether a user will interact with an item is not only decided by the user' own preferences, and other factors can also affect the user interactions on items. For instance, when a TV show is recently launched, the huge amount of discussions can make users watch it though they are not fans of these shows. The temporary popularity is beyond the original attributes of users and items. This kind of information is called as \emph{contexts} \cite{adomavicius2011context,verbert2012context,RAZA201984}. According to \citet{dey2001conceptual}, context is defined as "any information that can be used to characterize the situation of an entity. An entity is a person, place, or object that is considered relevant to the interaction between a user and an application, including the user and applications themselves". Leveraging the context information, a lot of methods are proposed. \citet{10.1145/1864708.1864727} extend the 2-d matrix factorization model to multi-dimensional tensor factorization, where the user-item-context tensor is treated as a generalized matrix. \citet{rendle2010pairwise} also organize the tag contexts of items as a user-item-context tensor, and they propose a novel algorithm called pairwise interaction tensor factorization (PITF), where the Bayesian Personalized Ranking (BPR) model is used to optimize the ranking list to make sure the positive samples have higher scores than the negative samples. \citet{10.1145/2872427.2883006} propose context-aware LDA model to recommend news by modeling the distribution of multiple contexts such as tweets, emails, posts or users’ personal attributes. \citet{10.1145/2365952.2365979} suggests that the contextual information may vary with time and cannot be described by static factors. They use a LDA model to search the latent topics from frequent song tags and then use a $k$-th order Markov model \cite{brooks2011handbook} to capture the user's contextual states over time.

%   \item \textbf{Session-based (Sequential-based) Recommendation.} Traditional recommender systems have a critical drawback – they assume that users' long-term behavior history is recorded, hence the recommendation can be made by modeling these static records. However, in many services, users do not log in and they cannot be identified, which means we do not have access of their long-term behavior history. In this situation, it is of great importance to model the limited behavior in those anonymous short-term behavior sessions. Here, a session can be regarded as a short period during which several items are purchased \cite{wang2019survey}. Recent efforts on tackling session-based recommendation can be generally classified into two categories: (1) Item-level dependency modeling. This branch refers to the modeling of inter-item dependency within a session. Usually, the task is to predict the next item based on the last items occurring in this session. Markov chain-based methods \cite{shani2005mdp,eirinaki2005web} and RNN-based methods \cite{10.1145/3079628.3079670,chen2019air,hidasi2015session-based,10.1145/3269206.3271761,li2017neural} have the natural advantages of capturing the sequential dependency because that they are designed for the time-series data. Besides, various methods are proposed to capture the dependency of items. For example, there are pattern-based methods \cite{lin2002efficient,mobasher2001effective}, convolutional neural network (CNN)-based methods \citet{10.1145/3159652.3159656,yuan2019simple}, translation-based methods \cite{he2017translation}, memory network-based methods \cite{chen2018sequential,wang2018neural}, and attention network-based methods \cite{wang2018attention,zhang2019next,ren2020sequential}. (2) Session-level dependency modeling. In contrast to item-level dependency modeling, session-level dependency modeling considers the relationship between item pairs or item lists from two consecutive sessions. \citet{rendle2010factorizing} formulate a sequential basket recommendation problem, where a user buys a set of items at the same time, and a transaction consists of more than one items and the task is to predict the next set of items.

% \end{itemize}


% \subsection{New Scenarios and Challenges in Recommendation}

% \subsubsection{Context-aware Recommendation}
% Traditional recommender problems are viewed as a prediction problem. Given a user profile and historical interaction on items, the recommender system aims to predict the user's ratings (a score) on certain items, then it makes recommendations using the items with the highest scores. However, in real-world situations, the users' ratings are not only decided by users' preferences, and other factors can also affect the user interactions on items. For instance, when a TV show is recently launched, the huge amount of discussions can make users who are not fans of these shows watch it. The temporary popularity is beyond the attributes of users and items. This kind of information is called as \emph{contexts} \cite{adomavicius2011context,verbert2012context,RAZA201984}. According to \citet{dey2001conceptual}, context is defined as "any information that can be used to characterize the situation of an entity. An entity is a person, place, or object that is considered relevant to the interaction between a user and an application, including the user and applications themselves". 

% To describe the additional information beyond user-item interaction, the pioneer work of \citet{adomavicius2011context} classify the context information into three classes: fully observable, partially observable, and unobservable. Then, according to the form of the context, they further divided all contexts into static context and dynamic context. They propose three intuitive frameworks for dealing with these contexts: (1) Contextual prefiltering, where the contexts are used to select the most relevant users and items. So a classic recommendation method can be used on the filtered user-item data.  (2) Contextual postfiltering, which ignores the context information in building recommendation models. Contexts are used to filter out the irrelevant results and adjust the ranking list. (3) Contextual Modeling. Instead of serving as a filter, contexts are directly considered into the model, so the model becomes the function of users, items, and contexts at the same time.

% The third way draw a lot of attention and a lot of methods are introduced. \citet{10.1145/1864708.1864727} extend the 2-d matrix factorization model to multi-dimensional tensor factorization, where the user-item-context tensor is treated as a generalized matrix. \citet{rendle2010pairwise} also organize the tag contexts of items as a user-item-context tensor, and they propose a novel algorithm called pairwise interaction tensor factorization (PITF), where the Bayesian Personalized Ranking (BPR) model is used to optimize the ranking list so that the positive samples have the higher scores than the negative samples. \citet{10.1145/2872427.2883006} propose context-aware LDA model to recommend news by modeling the distribution of multiple contexts such as tweets, emails, posts or users’ personal attributes. \citet{10.1145/2365952.2365979} suggests that the contextual information may vary with time and cannot be described by static factors. They use a LDA model to search the latent topics from frequent song tags and then use a $k$-th order Markov model \cite{brooks2011handbook} to capture the user's contextual states over time. 

% Point-of-Interest (POI) recommendation aims to recommend suitable places, e.g., restaurants and parks, for users to drop a visit \cite{yin2013lcars,gao2019bloma,yin2016discovering}. This branch of methods take the geographic information as contexts to constrain the model. The intuitive idea is to recommend the places nearby the user's current position. In social recommendation, the social network is used for assisting the recommendation. Unlike \acl{CF} algorithms, where other users having similar preferences with the target user is leveraged, social recommendation methods directly use the social network to assist recommendation. It assumes users' preference could be influenced from their friends' preferences, so many methods are proposed to extract items from their friends' purchase history as recommendation candidates. \cite{yu2018adaptive,yu2019generating}. Contextual information is also used in the bandit-based algorithm to enhance the decision process \cite{li2010contextual}. We will introduce the bandit problem in conversational recommender system later.

% \subsubsection{Session-based (Sequential-based) Recommendation}
% Traditional recommender systems have a critical drawback–they assume that users' long-term behavior history is recorded, so the recommendation can be made by modeling these static records. However, in many services, users do not log in and they cannot be identified, which means we do not have access of their long-term behavior history. In this situation, it is of great importance to model the limited behavior in those anonymous short-term behavior sessions. Here, a session can be regarded as a short period during which several items are purchased \cite{wang2019survey}. Recent efforts on tackling session-based recommendation can be generally classified into two categories: 

% \begin{itemize}
%     \item \textbf{Item-level dependency modeling}. This branch refers to the modeling of inter-item dependency within a session. Usually, the task is to predict the next item based on the last items occurring in this session. Markov chain-based methods \cite{shani2005mdp,eirinaki2005web} and RNN-based methods \cite{10.1145/3079628.3079670,chen2019air,hidasi2015session-based,10.1145/3269206.3271761,li2017neural} have the natural advantages of capturing the sequential dependency because that they are designed for the time-series data. Besides, various methods are proposed to capture the dependency of items. For example, there are pattern-based methods \cite{lin2002efficient,mobasher2001effective}, convolutional neural network (CNN)-based methods \citet{10.1145/3159652.3159656,yuan2019simple}, translation-based methods \cite{he2017translation}, memory network-based methods \cite{chen2018sequential,wang2018neural}, and attention network-based methods \cite{wang2018attention,zhang2019next,ren2020sequential}.
    
%     \item \textbf{Session-level dependency modeling. } In contrast to item-level dependency modeling, session-level dependency modeling considers the relationship between item pairs or item lists from two consecutive sessions. \citet{rendle2010factorizing} formulate a sequential basket recommendation problem, where a user buys a set of items at the same time. So a transaction consists of more than one items and the task is to predict the next set of items. They propose the FPMC model, whose core idea is to model the sequential set data as a  Markov chain, and the parameters simplified with the proposal of pairwise interaction. Then a general optimization criterion–sequential BPR (S-BPR) is proposed to optimize the maximum likelihood estimates on the sequential ranking model. Furthermore, there are neural network algorithms proposed to predict the items in the next basket \cite{wang2015learning,liu2018stamp,10.1145/3109859.3109896,yu2016dynamic,ying2018sequential}.
% \end{itemize}

% Also, there are methods considered exploring the item features to tackle the cold-start problem. these features can be referred as the contexts that we mentioned above \cite{10.1145/3109859.3109900,10.1007/978-3-319-71246-8_18,10.1145/2959100.2959156}.

% \subsubsection{Explainable Recommendation} 
% Existing recommender systems only pursue the accuracy of recommendation, while neglecting one of the most important tasks: exploring the reasons behind the recommendation results. Explainable recommendation focuses on the problem of why a recommendation is made. As \citet{ribeiro2016should} mentioned, if the users do not trust a model or a prediction, then they will not use it. The simple example of recommendation used in industry is the "people also viewed" explanation on the Amazon's product page. It is a direct description of the colleborative filtering result. 

% \citet{Zhang_2020} carry out a comprehensive overview of explainable recommendation. They classify the  existing explainable recommendation research into six categories based on the display style of the generated explanations: relevant user or item \cite{herlocker2000understanding,abdollahi2017using,heckel2017scalable,chen2018sequential,peake2018explanation,catherine2017explainable}, user profile or item features \cite{mcauley2013hidden,he2015trirank,vig2009tagsplanations,huang2018improving,seo2017interpretable}, a piece of textual sentence \cite{zhang2014explicit,ai2018learning,costa2018automatic}, visual image-based explanation \cite{10.1145/3331184.3331254,chen2018visually}, social factor explanation \cite{sharma2013social,ren2017social,park2017uniwalk}, and word cluster \cite{zhang2015incorporating,wu2015flame}. 

% Unlike these work that focus on providing a direct description or visualization to help user understand the pros/cons of the recommended items, some work aims to explain the model mechanism which is designed as a black box. \citet{zhang2014explicit} enrich meanings to the latent factor of matrix factorization model. Specifically, they extract explict product features from textual user reviews, and align each latent dimension in matrix factorization with a particular explicit feature, so that the factorization/prediction procedure can provide explicit explanations for the recommendations, e.g., "The mobile phone is recommended because you are interested in the quality of battery, and this product performs well on battery life". In addition, \citet{gao2019bloma} propose to use local rank-one matrix factorization to capture the maximum component of the residue matrix, and they align this component vector with item categories such as restaurants or parks. After repeating this process, they obtain a recommender system that can make recommendations accompanied by explanation like "This recommendation is tailored to your tastes for Chinese cuisine (fitting 60\%) and seafood (fitting 30\%)". \citet{wang2020disentangled} use a dynamic neighbor routing mechanism to automatically enrich a interaction behavior with one or multiple intents. For instance, "A man purchase a dress in a mall is because he wants to (1) pass the time, (2) shop for others". Besides, there are other works aimed at explaining the internal mechanism of the recommendation model. These techniques vary with the recommendation models and the perspectives of explanation.

\subsection{Challenges in Recommender Systems}
\label{secsub:challenges}
\subsubsection{The Cold-start Problem} 
A well-known problem in recommender systems is to handle new users or new items that barely appear in the training set. \Acf{CF} methods cannot handle such data; without historical data, it is impossible to find similar neighbors. For cold users, the most straightforward strategy is to recommend popular items, which turns out to be an effective strategy that is adopted by many kinds of recommender systems. It is a safe way since popular items have the maximal probability of attracting users with unknown preferences. However, this move will result in ``the rich get richer,'' i.e., popular items become more popular, while items with little attention will remain unexplored. In other words, the cold items will keep cold, even though they might be of great quality. The exploration and exploitation (E\&E) tradeoff is meant to address this issue, and we will discuss it in Session~\ref{sec:EE}. Another way to tackle this problem is to collect user profiles and item features, and feed them into content-based or context-based recommendation methods. This may be intractable in real-world scenarios since collecting data is expensive. The proposal of conversational recommender systems addresses this problem head on, as conversational systems can collect cold users' profiles and elicit preferences through interactions. Even though initially inferred preferences may be mistaken, the system can adjust its estimates after obtaining feedback.


\subsubsection{Fairness-aware Recommendation}
As we mentioned above, unbalanced data may result in a bias towards popular users or popular items. Unbalanced data may cause a model to get stuck in a local optimum, and it may bring unfair discrimination for a minority of users in terms of gender, race, ethnicity, religion, and so on. For example, when an Asian user resorts to an online job-matching system for seeking job opportunities in Europe, but since the system possesses user data that mainly consists of Europeans, the Asian user may not be able obtain the exposure and opportunities he deserves. This is not a deliberate manipulation of anyone, and the unfairness is caused by intrinsic imbalance in the data. There have been, and continue to be, many efforts to address this problem \cite{khademi2019fairness,zhu2018fairness,farnadi2018fairness,corbett2017algorithmic,geyik2019fairness,beutel2019fairness}. For example, \citet{geyik2019fairness} observe the issue of fairness in the LinkedIn ecosystem and use causality theory to detect whether a group of individuals that share sensitive attributes, e.g., race, gender, have been subjected to the discrimination of the system. \citet{zhu2018fairness} assume that  unfairness is accompanied by sensitive features such as gender or age. Therefore, they aim to isolate the sensitive information from the model representation and to derive the unbiased model. \citet{beutel2017beyond} propose focused learning, which uses different magnitudes of regularization on the majority group and the minority group, so as to increase the attention for the minority group. While the work just listed can help to mitigate the fairness issue, there is still a long way to go for eliminating the unfairness in recommendation models.

\subsubsection{Robustness}
As recommender systems have become key ingredients of complex financial revenue models, they have become a target for malicious manipulations. Malicious manipulations take advantage of the vulnerabilities of recommender systems. These vulnerabilities include a core principle underlying modern recommender systems, namely the ``wisdom of the crowd'' idea, with a view to increase or decrease the rating of certain items. This kind of manipulation is called a \emph{shilling attack}. Common strategies of shilling attack include random, average, popular, bandwagon, and love-hate attacks \cite{deldjoo2020dataset}. There are two kinds of strategies to resist the shilling attack. One is to directly detect and block fraudsters from the data \cite{aktukmak2019quick,chirita2005preventing,mobasher2007toward,mehta2009unsupervised}, and another is to increase the robustness of recommendation models under  shilling attacks \cite{huber2004robust,mehta2007robust}. For instance, \citet{he2018adversarial,tang2019adversarial} indicate that the recommender itself might be vulnerable to the perturbation of the input data. Hence, they propose to use adversarial training on the input data to improve the robustness of models. Furthermore, \citet{zhang2020gcn} combine the two strategies by proposing a GCN-based framework, where the task of fraudster detection and robust recommendation may benefit.


\subsubsection{Explainability of Recommendations} 
Existing recommender systems primarily focus on improving the accuracy of recommendations, while neglecting another important task: exploring the reasons behind the recommendation results. \emph{Explainable} recommendation focuses on the problem of idenitfying and explaining why a recommendation is made. A simple example of a recommendation used in industry is the ``people also viewed'' explanation on a product page. It is a direct description of the \acl{CF} result. 

\citet{Zhang_2020} carry out a comprehensive survey of explainable recommendations. They classify existing explainable recommendation research into six categories based on the display style (e.g., visual image-based explanation \cite{10.1145/3331184.3331254,chen2018visually}, social factor explanation \cite{ren2017social}, and textual-sentence-based explanation \cite{zhang2014explicit,zhang2015incorporating}) of the generated explanations.
% relevant user or item \cite{herlocker2000understanding,abdollahi2017using,heckel2017scalable,chen2018sequential,peake2018explanation,catherine2017explainable}, user profile or item features \cite{mcauley2013hidden,he2015trirank,vig2009tagsplanations,huang2018improving,seo2017interpretable}, a piece of textual sentence \cite{zhang2014explicit,ai2018learning,costa2018automatic}, visual image-based explanation \cite{10.1145/3331184.3331254,chen2018visually}, social factor explanation \cite{sharma2013social,ren2017social,park2017uniwalk}, and word cluster \cite{zhang2015incorporating,wu2015flame}. 
% relevant user or item, user profile or item features, a piece of textual sentence, visual image-based explanation, social factor explanation, and word cluster. 
Unlike studies that focus on providing a direct description or visualization to help users understand the pros and cons of the recommended items, some work aims to explain the model mechanism which is designed as a black box. For instance, 
% \citet{zhang2014explicit} enrich meanings to the latent factor of matrix factorization model. Specifically, they extract explicit product features from textual user reviews, and align each latent dimension in matrix factorization with a particular explicit feature. Thus, the factorization/prediction procedure can provide explicit explanations for the recommendations, e.g., "The mobile phone is recommended because you are interested in the quality of battery, and this product performs well on battery life". In addition, 
\citet{gao2019bloma} propose to use local rank-one matrix factorization to capture the maximum component of the residue matrix, and they align this component vector with item categories such as restaurants or parks. After repeating this process, they obtain a recommender system that can make recommendations accompanied by an explanation like ``This recommendation is tailored to your tastes for Chinese cuisine (fitting 60\%) and seafood (fitting 30\%).'' \citet{wang2020disentangled} use a dynamic neighbor routing mechanism to automatically enrich interaction behavior with one or multiple intents. For instance, ``A man purchases a dress in a mall because he wants to (1) pass the time, (2) shop for others.'' There is other works aimed at explaining the internal mechanism of the recommendation model; these techniques vary with the recommendation models and the target of the explanation.

% Though explainable recommendation has been explored in many works, there are problems and challenges remained. The first problem is that explainability is a wide concept, and different works have different probing directions, which are not even fall in a same research topic. Research in this field relies on the specific situation and certain model, and there is barely no standard metric for comparing different works. The second problem is more realistic: introducing of explainability in the model will compromise the model performance. This reason is natural, because the explainability is independent of accuracy, and it serves as a form of constraint in the original model.

It is worth mentioning that \acp{CRS} naturally support explainability. In a \ac{CRS}, the system can ask users for unsure facets to improve the reasoning mechanism, and it can make a recommendation accompanied by an explanation in the form of natural language \cite{chen2020ijcai}.
Explainability is an essential property of \acp{CRS}. From the model's perspective, capturing users' interests and intention becomes easy, which facilitates the recommendation process; from the user's perspective, they can understand how a recommendation is generated through the interaction, as a result of which users may be more likely to trust and rely on the system; from the developer's perspective, explanations can help debug and improve the model; and decision-makers can adjust their business strategies based on the explainable results.

\medskip\noindent%
Finally, there is a common challenge for most recommendation systems – eliciting user feedback. Requiring users to provide explicit feedback may hurt the user experiment since rating items is an onerous task for users. Besides, implicit feedback (e.g., click history or purchase records) is noisy because users may not actually like the item they interacted with or purchased. 
\acp{CRS} address this challenge, as we will discuss in \mysec{question-driven}.


% \subsection{Conversational Recommender Systems}
% Recently, conversational recommender system has drawn a lot of attention. Unlike other traditional recommender systems, CRS can interact with users, i.e., it can not only make recommendations, but also respond to users' feedback. This dynamics makes machines more like human beings, and it can be the possible pathway to the strong artificial intelligence.

% There is no widely accepted definition of CRS. \citet{nie2020workshop} borrow the concept of conversational search system \cite{radlinski2017theoretical} and formulates the definition of CRS as: 

% \emph{A system for recommendation that permits a mixed-initiative back and forth between a user and agent, where the agent’s actions are chosen in response to a model of current user needs, and about the store of information/products, within the current conversation, using both short- and long-term knowledge of the user.}

% The success of CRS is largely duo to the conversational component (i.e., the dialoge system), which is in the spotlight in the natural language processing community. Before the emerging of dialog systems, researchers have realized the importance of collecting users' real-time feedback in recommender systems. Researchers proposed the critiquing-based recommender system, which can be seemed as the earliest form of CRS \cite{tou1982rabbit,tversky1993context,burke1997findme,smyth2003analysis,pu2004decision,chen2012critiquing}. Critiquing in a recommender system is like a salesperson who will provide recommendation items based on users' current preference, which is collected by eliciting users to answer certain questions or actively choose from few predefined options with respect to specific attributes about items. For example, when seeking a mobile phone in the system, user may follow the hint of the system and provide information such as "I want something cheaper" or "I want the battery life to be longer". Based on these precious feedback, the system will retrieve the most possible items and return it to users, and the procedures can be repeated for several times until users find their satisfactory items or quit after losing patience.

% Through effective, the critiquing methods are constrained by its representation ability since users can interact with the system through predefined options (e.g., ticking checkboxes). The integrating of dialogue systems overcome this drawback, and the interaction between users and the system is in the form of natural language, which makes the interaction infinite possibilities. Generally, CRS can be formulate as a task-oriented dialogue system, where the task lies in two aspects: (1) to obtain information as precise as possible, (2) to satisfy users by recommending items. The general framework of CRS in task-oriented dialogue system includes three modules: Language understanding and generation module, dialgoue policy management module, and the core recommender engine.

% When building a intelligent CRS, we will encounter a lot of difficulties in each of the three components. We summary them into four key challenges:

% \begin{itemize}
%     \item \textbf{Making question-driven strategies.} The advantage of CRS is the opportunity to elicit user preferences by asking questions, so the model can modify its strategies based on user responds. If a user is satisfactory with the current recommendation, then the recommendation procedure stops there. Even an unsatisfactory item can play a useful role in articulating the user's goals. Thereby, it is of great importance to build a sophisticated multi-turn dialogue strategy which can sufficiently exploit the information in the question-driven dialogues.
%     \item \textbf{Handling language understanding and generation.} Through the language understanding and generation modules only need to handle the input and output of the recommender systems, it remains to be one of the hardest challenges in CRS. First, it is hard for machines to extract the accurate intent from user utterances, which could render disastrous results. To solve this issue, most CRS models use 
%   a common technique in task-oriented dialogue systems, i.e., slot filling, to project the user intention into several predefined attribute categories. We will describe in the next section. Besides, users' intention usually expresses in multiple turns of dialogues, and how to keep CRS consistent in multiple turns is also a tricky challenge.
%     \item \textbf{Trading off exploration and exploitation.} As mentioned earlier, one problem of recommender systems is the exposure of certain items could strengthen the trend of keeping recommending these items, while disregarding the unexplored items. Actually, these cold items can have high quality and recommending them to appropriate users can improve user experience. Bandit algorithms is tailored for this exploration and exploitation problem, and we will describe it later. Bandit algorithms require real-time interaction environment, which is exactly what CRS provides.
%     \item \textbf{Designing suitable evaluation metrics.} All three components need their own evaluation metrics. Besides evaluating the performance of the recommender engine using the common recommendation metrics (e.g., precision, recall, and hit rate), there if of great essence to evaluate the rest two dialogue related components. For instance, how much is the user intent understood by the language understanding module? Is the generated output consistent with last several turns of utterances? Would users feel bored in answering the multi-turn questions? To answer these question, there are several evaluation metrics proposed in CRS.
% \end{itemize}

% \begin{figure*}[!t]
% \centering
% \includegraphics[width=.8\linewidth]{figures/framework.pdf}
% \caption {Illustration of the general framework of conversational recommendation system and four key challenges.}
% \label{fig:framework}
% \end{figure*}

% Fig. \ref{fig:framework} illustrates the general frawework of CRS, and the four challenges is list in their corresponding components. We will discuss the four critical challenges in the following sections, with the hope of inspiring readers to break through the bottleneck of CRS. But first, we introduce the preliminaries of dialogue systems in the next section.


==> sections/removed-03-dialogue-systems.tex <==
\section{Introduction of Dialogue Systems}
\label{sec:DS}

Dialogue systems can be roughly divided into two classes: task-oriented dialogue systems and chatbots. Task-oriented dialogue systems are designed for fulfilling certain tasks such as booking restaurants or answering questions in certain domains. Chatbots, also known as non-task-oriented dialogue systems, aim to converse seamlessly and appropriately with human beings, and they often serve as a kind of entertainment. We illustrate the two kinds of dialogue systems in \myfig{ds} and describe the two branches in more detail below.

\tabcolsep=1pt
\begin{figure}[pos=t]
\centering
% \begin{tabular}{cc}
% \multicolumn{2}{c}{\includegraphics[width=0.9\linewidth]{figures/ds.pdf} }\\
% (a) Age and gender on Movie data  &   (b) Age and country on Book data
% \end{tabular}
\includegraphics[width=1\linewidth]{figures/ds_d.pdf}
\caption {Illustrations of the two main categories of dialogue systems.\mdr{It's not clear to me how this illustrates the two types of dialogue systems. Answer: We are considering remove this sections, Wenqiang Lei will consult with you soon.}}
\label{fig:ds}
\end{figure}


\subsection{Task-oriented dialogue systems}
Task-oriented dialogue systems use natural language to communicate with human beings for completing certain tasks. To achieve this, they usually consists of four components, i.e., a natural language understanding (NLU) module, a dialogue state tracking (DST) module, a dialogue policy learning module, and a natural language generation (NLG) module. The DST and dialogue policy learning component can merge to one part called the dialogue manager (DM) module \cite{chen2017survey,zhang2020recent}. The NLU, DST, and NLG components are often trained individually in advance, while the dialogue policy, which determines the decision-making process, is trained in the composed system.

\begin{itemize}[nosep,leftmargin=*]
    \item \textbf{Natural Language Understanding.} Traditional methods have two tasks, at different levels, to address when attempting to understand the user query. The low-level task is to extract keywords from the user's utterance and fill those into pre-defined semantic slots. A slot is a key-value pair such as ``\textit{Location: Beijing}'' or ``\textit{Color: Red}.'' Slot filling is defined as a sequence labeling problem, where words in a user's utterances are assigned with labels. Commonly used methods including deep belief networks (DBNs) \cite{deng2012use,deoras2013deep} and recurrent neural networks (RNNs) \cite{yao2013recurrent,mesnil2013investigation,yao2014spoken}. The other, high-level task is to categorize the intent of users, such as ``to find a restaurant'' or ``seeking music.'' 
    Deep learning techniques, which have been proved successful on classification problems, are widely used in this intent detection task \cite{deng2012use,yann2014zero,huang2013learning,shen2014learning,hashemi2016query}.
    
    \item \textbf{Dialogue State Tracking.} Since user intents cannot only be represented in one user utterance, tracking dialogue states is very important. At each timestamp, a dialogue state is detected and recorded. Many studies represent the dialogue state as a belief state, which is several probability distributions over the value vocabulary of each slot \cite{henderson2014second,williams2012belief}, thus it can be solved by statistical approaches \cite{wang2013simple,lee2013recipe,ren2013dialog,williams2013multi,williams2014web}. Recently, researchers have developed neural network-based methods to detect slot-value pairs \cite{henderson2013deep,mrksic-etal-2015-multi,mrksic-etal-2017-neural,10.1145/3394592}.
    
    \item \textbf{Dialogue Policy Learning.} The policy learning component is responsible for making decisions about which action to take based on the recorded states. The problem is often formulated as a Markov decision process (MDP), where an agent chooses an action based on the current state, and adjusts its action selecting policy according to the accumulated reward \cite{cuayahuitl2015strategic}. It should be noted that this method requires real-time user interactions, which is very expensive to collect \cite{Adiwardana2020TowardsAH}. To overcome this problem, many studies use simulated users to train the model \cite{li2017learning,10.1145/3314183.3323680,li-dialogue-2019,chen2020ijcai}. We will introduce user simulation techniques in \mysec{evaluation}.
    
    \item \textbf{Natural Language Generation.} As the last part of dialogue system, the NLG component directly determines the user experience. The generated utterance should not only convey the semantics of a dialogue act for task-completion, but also be natural, specific, and informative \cite{zhang2020recent}. Early methods generate the response by mapping key information to a tree-like structure, then outputting human-readable sentences via surface realization, which assures that the sentences will comply with the lexical and grammatical constraints \cite{walker2002training,stent-etal-2004-trainable}. Neural network-based methods have also been introduced in NLG because of their modeling abilities \cite{wen-etal-2015-semantically,10.1145/3394592,zhou2020improving,nips18/DeepConv}.
    % For example, \citet{wen-etal-2015-semantically} propose a LSTM-based model to take into account the dialogue act type and the slot-value pairs as the one-hot control input, which guarantees the responds to contain the intended meaning. \citet{10.1145/3394592} adopt adversarial reinforcement learning to directly reduce the difference between human responses and generated responses.
\end{itemize}

\noindent%
Furthermore, some studies aim to develop a fully data-driven neural network-based framework, in which the four components in traditional task-oriented dialogue systems are condensed into an end-to-end neural model. Unlike more traditional \ac{NLP} pipelines, which organize knowledge in different levels, e.g., phonology, morphology, syntax, semantics, and reasoning \cite{jurafsky2000speech}, neural approaches learn in a task-specific latent vector space. \citet{gao2019neural} summarize the learning procedure in three steps: 
\begin{enumerate*}[label=(\arabic*)]
\item encoding symbolic user input and knowledge into neural semantic representations, where semantically related or similar concepts are represented as vectors that are close to each other; 
\item reasoning in the neural space to generate a system response based on input and system state; and 
\item decoding the system response into a natural language output in a symbolic space. 
\end{enumerate*}
Since the three steps are implemented using an end-to-end neural framework,  explainability may be a point of concern as the model output is hard to interpret. 

Some researchers formulate their \ac{CRS} models as a task-oriented dialogue system, where the task is to recommend items to users \cite{nips18/DeepConv,chen-etal-2019-towards,Liao18mm}. However, in \acp{CRS}, the core task is to improve the recommendation performance and improve the user experience. Moverover, the standard dialogue modules may not be required for a \ac{CRS} model: the conversation mechanism can be represented in many forms, including in the form of tags or template utterances \cite{zhang2018towards,lei20estimation,lei2020interactive}.


\subsection{Chatbots}
Unlike task-oriented dialogue systems, chatbots do not have to fulfill a specific task; they need to meet the goal of chatting like a human. 
Given a user query, the system needs to provide a response. There are two ways of providing the response: using retrieval-based methods or generation-based methods.

\subsubsection{Retrieval-based Chatbots}
Retrieval-based chatbots are intuitive and they have been adopted by a lot of early research. The basic idea is to retrieve the appropriate response from a large collection of template response data. This problem can be formulated as a matching problem between an input user query and the candidate responses. The most straightforward method is to measure the inner-product of the feature vectors representing a query and a response, which is also referred to as single-turn response selection \cite{wu2019deep}. 

In single-turn response selection methods, the key problem is to learn a proper feature representation \cite{yan2018chitty}. One strategy is to use neural networks to learn the representation vectors from user query and candidate response, respectively. Then, a matching function is used to combine the two representations and output a matching probability \cite{hu2014convolutional,tan2016improved,qiu2015convolutional,feng2015applying,wang2016inner}. For example, \citet{hu2014convolutional} use a convolutional neural network for representation learning and a multiple layer perceptron network as the matching function. \citet{tan2016improved} use a bidirectional LSTM model for representation learning and the cosine function for matching learning. An alternative strategy, in contrast, is to combine the representation vectors of query and response first, and then a neural method is used on the combined representation pair to further learn the interaction \cite{wang2016learning,10.5555/3016100.3016298,10.5555/3016100.3016292,lu2013deep}. These two strategies have their own advantages: the former is more efficient and suitable for online serving, while the latter is better at efficacy since the matching information is sufficiently preserved and mined \cite{wu2019deep}.

The methods mentioned above are designed for retrieving a single response with regard to the current turn of user utterances. However, in real-world conversations, it is rare for users to articulate their intention in a single utterance. Hence, the model needs to consider exploiting the context, i.e., the last several turns of user utterances, to better understand the user intention and produce consistent responses. Such multi-turn response selection methods \cite{wu2019deep} match the candidate response with multiple turns of user utterance, instead of one, at the same time. According to \citet{wu2019deep}, there are also two strategy frameworks, just like in the single-turn response selection, to learn the matching between queries and the candidate responses \cite{lowe-etal-2015-ubuntu,zhou2016multi,yan2016learning,wu-etal-2019-sequential,wu2019sequential}.


\subsubsection{Generation-based Chatbots}

Another way to produce responses is through gener\-ation-based methods. Unlike retrieval-based methods, which select existing responses from a database of template response, generation-based methods use the language generation techniques in \ac{NLP}. The basic generation model is a recurrent sequence-to-sequence model, which sequentially feeds in each word in the query as input, and then generates the output word one by one \cite{sutskever2014sequence}. The sequence-to-sequence response generation methods can also be divided into single-turn response generation \cite{ritter2011data,shang-etal-2015-neural,vinyals2015neural} and multi-turn response generation which uses context information \cite{sordoni-etal-2015-neural,serban2016building,tian-etal-2017-make}.

Compared to retrieval-based methods, generation-based methods have some challenges. First, the generated answer is not guaranteed to be a well-formed natural language utterance \cite{yan2016learning}. Second, even though the generated response may be grammatically correct, we can still distinguish a machine-generated utterance from a human-generated utterance, since the machine response lacks basic commonsense \cite{young2018augmenting,zhou2018commonsense}, personality \cite{ijcai2018-595} and emotion \cite{zhou2018emotional}. Even worse, generation models are prone to produce a safe answer, such as ``OK,'' ``I don't understand what you are talking about,'' which can fit in almost all conversational contexts but would only hurt the user experience. \citet{ke-etal-2018-generating} propose to explicitly control the function of the generated sentence, for example, for the same user query, the system can answer with different tones: The interrogative tone can be used to acquire further information; the imperative tone is used to make requests, directions, instructions or invitations to elicit further interactions; and the declarative tone is commonly used to make statements or explanations. Another problem is how to evaluate the generated response, since there is no standard answer; we will further discuss this in mysec{evaluation}.

Chatbots aim to converse with human beings with rational, consistent, and fluent language. To achieve that, most models try to directly learn from human utterances of a collected dataset to produce appropriate responses. However, real-world dialogues can be tactical and rely on the situation. Therefore, some researchers propose to enrich them with chatting tactics such as the ability to negotiate \cite{lewis-etal-2017-deal} or persuade \cite{wang-etal-2019-persuasion}. These techniques are also useful in \acp{CRS}, which can improve the user experience beyond mere user-item interactions.

